Data Race Detection by Digest-Driven Abstract Interpretation (Extended Version)

Sound static analysis can prove the absence of data races by establishing that no two conflicting memory accesses can occur at the same time. We repurpose the concept of digests -- summaries of computational histories originally introduced to bring tunable concurrency-sensitivity to thread-modular value analysis by abstract interpretation, extending this idea to race detection: We use digests to capture the conditions under which conflicting accesses may not happen in parallel. To formalize this, we give a definition of data races in the thread-modular local trace semantics and show how exclusion criteria for potential conflicts can be expressed as digests. We report on our implementation of digest-driven data race detection in the static analyzer Goblint, and evaluate it on the SV-COMP benchmark suite. Combining the lockset digest with digests reasoning on thread ids and thread joins increases the number of correctly solved tasks by more than a factor of five compared to lockset reasoning alone.

==> content/tailored-digests/non-content/once.tex <==
\subsection{Synchronization via \texttt{pthread\_once}}\label{ss:once}

The \pthreads\ library offers a mechnism for executing a given operation at most once.
%
This is helpful, e.g., for initializing a resource before any thread can access it.
%
Examples include opening a log file for writing or creating a database connection that is to be shared among threads.
%
While a developer writing a program would usually place such code in the \texttt{main} function,
this option is not available to library developers~\cite{butenhof1993programming} as it is not them who write the main
function.
%
They instead rely on a dedicated mechanism---\texttt{pthread\_once}.

The \texttt{pthread\_once} mechanism provides a type for control variables (which we assume to be from some set $\mathcal{O}$) and a function
\texttt{pthread\_once(o,f)} which, if $o$ is not set, executes the function $f$ and sets $o$, and otherwise
does nothing. The system ensures that running $f$ and setting $o$ appears atomic to all threads.

\begin{figure}
    \begin{minipage}[t]{7cm}
\begin{minted}[tabsize=1]{c}
// Library file
pthread_once_t once;
schmilblick* dev; // Some device

void init_lib() {
  dev = malloc(size_of(schmilblick));
  init_schmilblick(dev);
}

void maluba(){
  // Ensure the library is initialized
  pthread_once(once,init_lib);
  assert(dev != NULL);
  // ...
}
\end{minted}
\end{minipage}\begin{minipage}[t]{7cm}
    \begin{minted}[tabsize=1]{c}
// Main file
void *t1(void *arg) {
  maluba();
  // ...
  return NULL;
}

int main() {
  pthread_ t t;
  pthread_create(&t, t1, NULL);

  maluba();
  // ..
}
    \end{minted}
        \end{minipage}
\caption{\textsc{Pthread} program using \texttt{pthread\_once}}\label{f:onceComplete}
\end{figure}
%
Consider the program in \cref{f:onceComplete}.
Here, the function \texttt{init\_lib} contains some library initialization code to allocate a device pointer and initialize
the device.
%
This code needs to be executed before any of the other library functions can be used. The library function \texttt{maluba} is
called from both the main thread and another thread. Here, \texttt{pthread\_once} is used to ensure that \texttt{init\_lib}
is called exactly once, and that the device pointer is initialized before it is used.

%
This feature is often overlooked by static analyzers or abstracted very crudely. With the help of digests, it
becomes possible to handle this feature more precisely without complicating the underlying analysis.
In fact, all the right-hand sides of an analyzer can return the abstract value corresponding to their first
argument here, all other handling happens inside the digest.
%
Nevertheless, two entire class of races, namely those between instructions in the function called by \texttt{pthread\_once}
as well as those between this initialization and other code executed later can be excluded.
%

\paragraph{Extension of the concrete semantics.}
To facilitate analysis, we introduce a new, observable, action $\onceInit(o)$ to initialize a control
variable $o$ at start of the program\footnote{
    This seems like it might negate the need for \texttt{pthread\_once}, but a static analyzer usually has the whole
    program at hand and can thus (conceptually) place helper code at the beginning of the program, while this
    is not true for library developers.
} and compile a call to \texttt{pthread\_once(o,f)} to a sequence first calling $\onceStart(o)$, then branching
on $\onceRan(o)$ and executing the (inlined) code from $f$ if $\onceRan(o)$ is false. Then, the operation $\onceEnd(o)$ is performed.
% In the concrete semantics, the branching on $\onceRan(o)$ inspects the local trace by checking for the presence of
% an % Needs to be an, macro expands to endOnce
% $\onceEnd(o)$ operation in the local trace.
%
Here, $\onceInit(o)$ and $\onceEnd(o)$ on the one hand, and $\onceStart(o)$ on the other form
pairs of observable and observing actions, as is the case for $\init(a)$, $\unlock(a)$ and
$\lock(a)$ for a mutex $a$.
In fact, for a control variable $o$ and these actions, the requirements on the once order $\to_{o}$ correspond exactly
to those on the mutex order $\to_{a}$ for some mutex $a$ as outlined in \cref{s:lt}.
The actions $\Pos(\onceRan(o))$ and $\Neg(\onceRan(o))$, i.e, the guards checking whether the code associated with
\texttt{pthread\_once} is to be executed, then return a local trace only in case an action $\onceEnd(o)$
appears somewhere in the trace, respectively when no such action appears in the local trace.\footnote{
Recursively calling \texttt{pthread\_once(o,f)} is not conclusively specified in the standard; Here,
we decided to go for the behavior of \texttt{glibc}, which deadlocks upon such calls.
}
%


Consider \cref{f:once}. This program corresponds to the one in \cref{f:onceComplete} when abstracting away
some details and expressing \textsf{pthread\_once} as a sequence of actions
as outlined above.

\begin{figure}
    \begin{minipage}[t]{7cm}
\begin{minted}[tabsize=1]{c}
main:
 initO(o);
 create(t1);
 ...
 startO(o);
 if(!ran(o)) {
    lock(m_dev);
    dev = malloc(42);
    unlock(m_dev);
 }
 endO(o);

 lock(m_dev);
 assert(dev != NULL);
 unlock(m_dev);

\end{minted}
    \end{minipage}\begin{minipage}[t]{7cm}
\begin{minted}[tabsize=2]{c}
t1:
 ...
 startO(o);
 if(!ran(o)) {
    lock(m_dev);
    dev = malloc(42);
    unlock(m_dev);
 }
 endO(o);

 ...

 lock(m_dev);
 assert(dev != NULL);
 unlock(m_dev);
\end{minted}
    \end{minipage}
\caption{Program highlighting how \texttt{pthread\_once} is decomposed into individual steps.}\label{f:once}
\end{figure}

A digest to help analyze this feature (\cref{f:onceASimple}) may then track two pieces of information in a tuple $(A,C)$:
\begin{itemize}
    \item Some set $A$ of \emph{active} control variables, i.e., those for which the ego thread currently is inside the section
    between $\onceStart(o)$ and $\onceEnd(o)$.
    \item Some set $C$ of \emph{completed} control variables, i.e., control variables for which the associated fragment
    has surly been run, as a call to $\onceEnd(o)$ was observed.
\end{itemize}
%
The guards $\Pos(\onceRan(o))$ and $\Neg(\onceRan(o))$ then check whether $o$ already has been completed, i.e., is in $C$ or not.
$\onceStart(o)$ adds the control variable $o$ to the active set, and $\onceEnd(o)$ removes it from the active set, but adds it to
the completed set.
%
\begin{figure*}[t]
    \begin{minipage}[t]{.5\linewidth}\[
        \begin{array}{lll}
        \Digests = 2^\Onces\times 2^\Onces\\[0.5ex]
		\initDigests = \{(\emptyset,\emptyset)\}\\[0.5ex]
        \newDigests\,(A,C)\,u\,u_1= \{(\emptyset,C)\}\\[0.5ex]
        \semDigests{\Pos(\onceRan(o))}\,(A,C) =\\
        \qquad \begin{cases}
            \emptyset & \text{if } \texttt{o} \not\in C\\
            \{ (A,C) \} & \text{otherwise}
        \end{cases}\\
        \semDigests{\act}\,(A,C) = \{(A,C)\} \quad \text{(other non-observing)}\qquad\;\;\\

        \semDigests{\act}\,(A_0,C_0)\,(A_1,C_1) = \{ (A_0, C_0)  \} \quad \text{(other observing)}\\
        \end{array}%
    \]
    \end{minipage}%
    \begin{minipage}[t]{.3\linewidth}\[
        \begin{array}{lll}
            \semDigests{\onceStart(o)}\,(A_0,C_0)\,(A_1,C_1) =\\
            \qquad \begin{cases}
                \{(A_0 \cup \{o\}, C_0 \cup C_1)\} & o \not\in A_0\\
                \emptyset & \text{otherwise}
            \end{cases}\\
            \semDigests{\onceEnd(o)}\,(A,C) = (A \setminus \{o\}, C \cup \{o\})\\[0.5ex]
            \qquad\qquad\semDigests{\Neg(\onceRan(o))}\,(A,C) =\\
            \qquad\qquad\qquad \begin{cases}
                \emptyset & \text{if } \texttt{o} \in C\\
                \{ (A,C) \} & \text{otherwise}
            \end{cases}
        \end{array}
        \]
    \end{minipage}
    \caption{Right-hand sides for excluding races based on \texttt{pthread\_once}.}\label{f:onceASimple}
\end{figure*}
%
% This only counts those as observed that came in via a start_once call. It is a bit odd but still a valid digest
% The motivation is from the analysis: making all other actions ego-lane-derived means we don't need to put anything on
% m_g variables
% The implementation is even cheekier and underapproximates c to those that have happened along the ego lane.
The race check predicate can then be defined as:
\[
(A,C)\;||^{?}\;(A',C') = \begin{cases}
    \textsf{false} & \text{ if } (A \cap (A' \cup C') \neq \emptyset ) \lor (A' \cap (A \cup C) \neq \emptyset)\\
    \top & \text{otherwise},
\end{cases}
\]
i.e., accesses where the same control variables are active may not race, and neither may accesses
where for one the control variable is active, and for the other it is completed.
%
\begin{example}
    Consider again the program in \cref{f:once}. An analysis using the digest from \cref{f:onceASimple}
    succeeds in establishing race freedom.
    $\hfill\qed$
\end{example}
%
In fact, an extended version of this digest can also make the analysis of values of global variables
% in programs using \texttt{pthread\_once}
more precise. We detail this in \cref{app:oncelong}.


==> content/tailored-digests/non-content/related.tex <==

\paragraph{Static Analysis of Barriers} Barriers have been studied
widely~\cite{le_verification_2013,mittermayr_kronecker_2016,kokologiannakis_bam_2021,murthy_design_2016},
also in the context of OpenMP \cite{Lin05,SwainLLLG020,SwainH18}, where their usage is usually well-structured.
Here, we focus on work on \pthreads-style barriers.
\citet{mittermayr_kronecker_2016} extend the use of Kronecker algebra from the static analysis of semaphores to barriers.
\citet{kokologiannakis_bam_2021} enhance the performance of stateless model checking by not distinguishing between interleavings that only differ in the order in which threads arrived at a barrier.
There, it is required that the initial capacity of a barrier is an upper bound to the number of \textsf{phtread\_barrier\_wait} calls that happen in parallel.
The analysis is justified w.r.t a semantics of concurrent programs on execution graphs.
\citet{murthy_design_2016} describe the design of a distributed phaser, a synchronization construct similar to Barriers
and verify the correctness of their implementation using the SPIN model checker.
They do not concern themselves with analyzing code using the construct.
%
\citet{le_verification_2013} propose a separation logic based verification technique for barrier synchronization
that employs bounded partial permissions to establish that a program is well-synchronized, by which they mean
that the program execution of all threads participating in a barrier can be partitioned into phases delineated
by calls to the barrier that proceed in lockstep. In this way, e.g., races between accesses located in
separate phases can be excluded.
% On top of the type of barrier found in \texttt{pthread} which we focus on, their work also consider barriers
% were the capacity may change during execution, as they can, e.g., be found in the \texttt{.NET framework}~\cite{dotnetbarriers}
% or in \texttt{Java} for \texttt{Phaser}s~\cite{phasersjava}.
Their approach relies on user-provided annotations with a reported annotation overhead of, on average, around 10\%.
\citet{HoborG2012} also propose a separation logic for programs using barriers.
Again, this verification approach relies on user-supplied annotations.
In contrast, our approach is fully automatic and does not require any annotations.
\citet{JeremiassenE94} propose an algorithm to determine which sections of processes of a program using barriers cannot run concurrently.
To this end, the execution of the program is conceptually split into phases divided by barriers.
The results of the algorithms are intended for the use in compilers to reduce \emph{false sharing} and thus the number of cache misses.

\paragraph{Static analysis of \texttt{pthread\_once}} The situation is different for \texttt{pthread\_once}: While missing support
has been mentioned as a limitation in
some works~\cite{SiegelZLZMEDR15, LeRVBDO22}, we are, to the best of our knowledge, the first to propose an analysis technique
for this feature that goes beyond
syntactical considerations~\cite{sonarsource}---whether in the context of race detection or static analysis in general.


==> figures/lockset-digest-example.tex <==
\begin{figure}
    \input{figures/program-mg-mutexes-running-example-lockset-digest.tex}
    \caption{The program in \cref{l:prog1} annotated using the digest in \cref{f:locksets}.}
    \label{l:prog1:lockset-digest}
    \vspace{1em}
\end{figure}


==> figures/threading-mode-digest-example.tex <==
\begin{figure}
    \input{figures/program-mg-mutexes-running-example-mt-digest.tex}
    \caption{The program in \cref{l:prog1} annotated with the digests found by an analysis using the digest in \cref{f:threadingmainA}.}
    \label{l:prog1:mt-digest}
    \vspace{1em}
\end{figure}

